Bandit Guided Submodular Curriculum for Adaptive Subset Selection

Traditional curriculum learning proceeds from easy to hard samples, yet defining a reliable notion of difficulty remains elusive. Prior work has used submodular functions to induce difficulty scores in curriculum learning. We reinterpret adaptive subset selection and formulate it as a multi-armed bandit problem, where each arm corresponds to a submodular function guiding sample selection. We introduce ONLINESUBMOD, a novel online greedy policy that optimizes a utility-driven reward and provably achieves no-regret performance under various sampling regimes. Empirically, ONLINESUBMOD outperforms both traditional curriculum learning and bi-level optimization approaches across vision and language datasets, showing superior accuracy-efficiency tradeoffs. More broadly, we show that validationdriven reward metrics offer a principled way to guide the curriculum schedule.

==> AuthorKit25/AnonymousSubmission/LaTeX/comments.tex <==
 
    \begin{comment}
        Our problem setting employs an adaptive subset selection
    and refinement strategy. In contrast to standard full mini-batch training, at
    each step $t$, the model is trained solely on a carefully selected subset
    $\mathcal{S}_{t}\subseteq \mathcal{B}_{t}$ of size
    $\beta = |\mathcal{S}_{t}| \ll |\mathcal{B}_{t}|$. This selective training aims to
    accelerate convergence \citep{revisit-micro-batch} while maintaining near-optimal
    test accuracy. To achieve this adaptive selection, we draw inspiration from
    the framework of online submodular optimization problems \citep{streeter2009online, salem2024online}.
    \end{comment}


==> AuthorKit25/AnonymousSubmission/LaTeX/old_experiments_details.tex <==

 \section{Experimental Setup}
    In order to showcase that $\methodprop$ performs better
    Our experiments aim to showcase the efficiency and accuracy tradeoffs of our
    proposed approach $\methodprop$ across a range of configurations and on a
    variety of datasets. We perform all our experiments on NVIDIA A6000s GPUs and
    to provide a fair comparison across all baselines. We share more details on
    the individual training cost in Appendix \ref{Appendix: Experiment Details}.


\subsection{Language Model Datasets}


\textbf{Model-Training-Evaluation Pairs.} We evaluate $\methodprop$ using combinations of three LLMs—\texttt{LLAMA-2-7B} and \texttt{MISTRAL-7B}—finetuned on LESS data, with performance assessed on MMLU and TYDIQA (Table 1).


\begin{table}[h!]
\centering
\caption{Performance comparison across tasks. Bold indicates best performance in each column.}
\vspace{0.5em}
\rowcolors{2}{gray!20}{white}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\rowcolor{gray!20}
\textbf{Method} & \textbf{Avg.} & \textbf{Soc.} & \textbf{Pol.} & \textbf{Hist.} & \textbf{Anat.} & \textbf{ML.} & \textbf{Eth.} & \textbf{Gen.} & \textbf{Bio.} & \textbf{Chem.} & \textbf{TydiQA} \\
\midrule
GradNorm        & 46.4\%          & 61\%          & 62\%          & \textbf{52\%}  & 40\%           & 40\%          & 43\%          & 46\%          & 42\%          & 32\%           & 54.6\% \\
MaxLoss         & 45.4\%          & 60\%          & 64\%          & 48\%           & 39\%           & 38\%          & 44\%          & 43\%          & 42\%          & 31\%           & 55.4\% \\
GREATS          & 47.8\%          & 63\%          & 66\%          & 48\%           & 42\%           & 41\%          & 46\%          & 48\%          & 43\%          & 33\%           & 55.4\% \\
\textbf{Ours}   & \textbf{49.8\%} & \textbf{64\%} & \textbf{67\%} & \textbf{52\%}  & \textbf{45\%}  & \textbf{42\%} & \textbf{48\%} & \textbf{50\%} & \textbf{45\%} & \textbf{35\%}  & \textbf{55.9\%} \\
\bottomrule
\end{tabular}
}
\end{table}





We compare our algorithm with regular training and a variety of online batch selection
algorithms: (1) MaxLoss [28], which selects training data points with the highest loss values. (2)
GradNorm [23], which prioritizes training data points with the highest gradient norms


\begin{figure}[htbp]
\centering

% === Figure 1 ===
\begin{minipage}[t]{\textwidth}
\centering
\scalebox{0.26}{%
\input{AuthorKit25/AnonymousSubmission/LaTeX/LLMs_results/tickz_test_pplx_astro_mmlu.tex}
}
\scalebox{0.26}{%
\input{AuthorKit25/AnonymousSubmission/LaTeX/LLMs_results/tickz_test_pplx_astro_mmlu.tex}
}
\scalebox{0.23}{%
\input{AuthorKit25/AnonymousSubmission/LaTeX/LLMs_results/tickz_test_pplx_astro_mmlu.tex}
}
\scalebox{0.23}{%
\input{AuthorKit25/AnonymousSubmission/LaTeX/LLMs_results/tickz_test_pplx_astro_mmlu.tex}
}
\end{minipage}

\caption{Test Perplexity Comparison Across Five MMLU Algorithm Baselines}
\end{figure}



\subsection{Vision Datasets}

   We showcase the utility of our method across 6 datasets primarily CIFAR-10, CIFAR100
    \citep{krizhevsky2009learning}, MNIST \citep{lecun2010mnist}, SVHN\citep{netzer2011reading},TinyImagenet\citep{le2015tiny}.
    For feature extraction for such image datasets, we utilize DINO\footnote{https://huggingface.co/facebook/dino-vitb16},
    chosen as per the findings of ablation study I1 in \cite{killamsetty2023milo}.
    For all our experiments we consider $\mathcal{K}= 5$ (consisting of \textit{FacilityLocation},
    \textit{GraphCut}, \textit{DisparityMin} \textit{DisparitySum} and \textit{LogDet}
    details pertaining to the same are provided in Appendix
    \ref{Appendix:SubmodDetails}).

    \textbf{Baselines for Comparison} We compare our proposed approach $\methodprop$
    with a variety of other notable benchmarks consisting primarily of the following:
   \blackcircle{1} $\baselineGradmatch$: \citep{killamsetty2021grad}, \blackcircle{2} $\baselinecraig$ \citep{mirzasoleiman2020coresets},
     \blackcircle{3} $\baselineglister$ \citep{killamsetty2021glister}, \blackcircle{4} $\baselinerho$ \citep{mindermann2022prioritized}
    and \blackcircle{5} $\baselineboss$ \citep{acharyabalancing}. A detailed summary of individual baselines are presented in Appendix section.

\textbf{Performance Metrics across all baselines} To compare various baselines,
    we utilize \textbf{Speedup} as a relative measure of the training times for each
    baseline in relation to full batch training. For \textbf{Relative accuracy},
    we define it as the accuracy achieved by the respective baseline on the test
    set compared to that of full batch training. Our goal is to identify a baseline
    that achieves both high speedup and high relative accuracy.

We showcase for both sample wise and batchwise settings in our experiments here
Since our proposed method is more suitable for in batch computation we compare against the \textit{PerBatch} variant of each of these models. We share the corresponding
    hyperparameter details in Appendix \ref{Appendix:Hyp}

Figure \ref{fig:batchwise_results} showcases the perbatch variant while Figure \ref{fig:samplewise_results} showcases for sample wise settings



  \begin{comment} 
    \begin{figure*}[h!]
        \centering
        \includesvg[width=0.8\textwidth]{grid.svg}
        \caption{Speed Up  vs Relative Test Accuracy ($\methodprop$-Batch \textbf{Batchwise
        version Perfomance}): ResNet18 models trained on batch size=128 with
        submodular budget fractions of 10\%(0.1), 30\%(0.3) and 50\%(0.5) respectively.$\methodprop$
        performs significantly well in comparison to other baselines both in terms
        speed up and relative test accuracy across 3 benchmark vision datasets}
        \label{fig:batchwise_results}
    \end{figure*}
  \end{comment}  


\begin{table}[h!]
\centering
\caption{Performance comparison across different datasets and fractions. Bold indicates the best performance in each column.
Speed Up  vs Relative Test Accuracy ($\methodprop$-Batch \textbf{Batchwise
        version Perfomance}): ResNet18 models trained on batch size=128 with
        submodular budget fractions of 10\%(0.1), 30\%(0.3) and 50\%(0.5) respectively.$\methodprop$
        performs significantly well in comparison to other baselines both in terms speed up and relative test accuracy across 3 benchmark vision datasets
        }
\vspace{0.5em}
\rowcolors{2}{gray!20}{white}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\toprule
\rowcolor{gray!20}
\textbf{Method} & \multicolumn{3}{c|}{\textbf{TinyImageNet}} & \multicolumn{3}{c|}{\textbf{CIFAR-100}} & \multicolumn{3}{c|}{\textbf{CIFAR-10}} \\
\cline{2-10}
 & \textbf{10\%} & \textbf{30\%} & \textbf{50\%} & \textbf{10\%} & \textbf{30\%} & \textbf{50\%} & \textbf{10\%} & \textbf{30\%} & \textbf{50\%} \\
\midrule
CRAIG & 0.82 / 4.82 & 0.858 / 2.41 & 0.96 / 1.7 & 0.938 / 2.5 & 0.947 / 6.7 & \cellcolor{yellow!50} \textbf{0.979} / 1.5 & 0.947 / 6.7 & 0.967 / 2.9 & 0.979 / 1.15 \\
MILO & 0.835 / 8.62 & 0.926 / 3.1 & 0.973 / 2.6 & 0.97 / 3.5 & 0.97 / 5.8 & 0.985 / 1.95 & 0.97 / 5.8 & 0.98 / 2.05 & 0.99 / \cellcolor{yellow!50} \textbf{2.15} \\
GRADMATCH & 0.812 / 5.92 & 0.906 / 2.62 & 0.968 / 2.1 & 0.963 / 3.1 & 0.969 / 4.3 & 0.98 / 1.3 & 0.969 / 4.3 & 0.98 / 1.95 & 0.99 / 1.48 \\
GLISTER & 0.803 / 5.5 & 0.875 / 2.65 & 0.971 / 1.7 & 0.938 / 2.6 & 0.957 / 4.5 & 0.971 / 1.2 & 0.957 / 4.5 & 0.968 / 1.7 & 0.974 / 1.3 \\
RHO & 0.845 / 5 & 0.922 / 2.57 & 0.97 / 2 & 0.974 / 1.9 & 0.945 / 2.5 & 0.985 / \cellcolor{yellow!50} 1.2 & 0.945 / 2.5 & 0.962 / 1.6 & \cellcolor{yellow!50} \textbf{0.988} / 1.15 \\
BOSS & 0.821 / 5.4 & 0.94 / 2.9 & 0.97 / 2.15 & 0.96 / 3 & 0.964 / 4.9 & 0.982 / 1.9 & 0.964 / 4.9 & 0.977 / 1.8 & 0.986 / 1.53 \\
ONLINESUBMOD & 0.862 / 8.43 & 0.937 / 3.08 & \cellcolor{yellow!50} \textbf{0.975} / 2.6 & 0.975 / 3.3 & 0.972 / 5.4 & 0.986 / 1.92 & \cellcolor{yellow!50} \textbf{0.972} / 5.4 & \cellcolor{yellow!50} \textbf{0.985} / 2 & \textbf{0.99} / 2.08 \\
\bottomrule
\end{tabular}
}
\end{table}




\begin{figure*}[h!]
        \centering
        \scalebox{0.83}{\input{AuthorKit25/AnonymousSubmission/LaTeX/plots_samplewise.tex}}
        \caption{\textbf{Samplewise version Performance} on CIFAR-10, CIFAR-100,
        SVHN, and Tiny ImageNet: $\methodprop$ performs better on average than other
        baseline counterparts across subset percentages}
        \label{fig:samplewise_results}
    \end{figure*}

\begin{comment}
\begin{table}[ht]
\centering
\captionsetup{font=small}
\caption{Test accuracy (\%) and training speedup (×) on TinyImageNet, CIFAR10, and CIFAR100 at 10\%, 30\%, and 50\% subset sizes. Each cell reports \texttt{accuracy / speedup}.}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{
    l
    >{\columncolor{LightBlue}}c
    >{\columncolor{LightBlue}}c
    >{\columncolor{LightBlue}}c
    >{\columncolor{LightGreen}}c
    >{\columncolor{LightGreen}}c
    >{\columncolor{LightGreen}}c
    >{\columncolor{LightOrange}}c
    >{\columncolor{LightOrange}}c
    >{\columncolor{LightOrange}}c
}
\toprule
\textbf{Method} 
& \multicolumn{3}{c}{\textbf{TinyImageNet}} 
& \multicolumn{3}{c}{\textbf{CIFAR10}} 
& \multicolumn{3}{c}{\textbf{CIFAR100}} \\
& 10\% & 30\% & 50\% & 10\% & 30\% & 50\% & 10\% & 30\% & 50\% \\
\midrule
FULL (skyline)          & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× & 64.36 / 1.0× \\
RANDOM (skyline)        & 19.61 / 6.4× & 35.68 / 3.1× & 43.84 / 2.0× & 19.61 / 6.4× & 35.68 / 3.1× & 43.84 / 2.0× & 19.61 / 6.4× & 35.68 / 3.1× & 43.84 / 2.0× \\
CRAIG                   & 52.42 / 6.4× & 55.56 / 3.1× & 61.48 / 2.0× & 52.42 / 6.4× & 55.56 / 3.1× & 61.48 / 2.0× & 52.42 / 6.4× & 55.56 / 3.1× & 61.48 / 2.0× \\
GLISTER                 & 51.54 / 6.4× & 56.37 / 3.1× & 62.15 / 2.0× & 51.54 / 6.4× & 56.37 / 3.1× & 62.15 / 2.0× & 51.54 / 6.4× & 56.37 / 3.1× & 62.15 / 2.0× \\
GRADMATCH               & 52.63 / 6.4× & 58.19 / 3.1× & 61.93 / 2.0× & 52.63 / 6.4× & 58.19 / 3.1× & 61.93 / 2.0× & 52.63 / 6.4× & 58.19 / 3.1× & 61.93 / 2.0× \\
MILO                    & 53.24 / 6.4× & 59.36 / 3.1× & 62.28 / 2.0× & 53.24 / 6.4× & 59.36 / 3.1× & 62.28 / 2.0× & 53.24 / 6.4× & 59.36 / 3.1× & 62.28 / 2.0× \\
RHO-LOSS                & 54.46 / 6.4× & 59.78 / 3.1× & 62.15 / 2.0× & 54.46 / 6.4× & 59.78 / 3.1× & 62.15 / 2.0× & 54.46 / 6.4× & 59.78 / 3.1× & 62.15 / 2.0× \\
BOSS                    & 52.63 / 6.4× & 60.17 / 3.1× & 62.13 / 2.0× & 52.63 / 6.4× & 60.17 / 3.1× & 62.13 / 2.0× & 52.63 / 6.4× & 60.17 / 3.1× & 62.13 / 2.0× \\
\textbf{ONLINESUBMOD (ours)} & \textbf{55.30 / 6.4×} & \textbf{60.74 / 3.1×} & \textbf{62.58 / 2.0×} & \textbf{55.30 / 6.4×} & \textbf{60.74 / 3.1×} & \textbf{62.58 / 2.0×} & \textbf{55.30 / 6.4×} & \textbf{60.74 / 3.1×} & \textbf{62.58 / 2.0×} \\
\bottomrule
\end{tabular}
}
\end{table}

\end{comment}

\subsection{Dataset details, model architecture setup}

   
    % \input{exponent_analysis.tex}

    \begin{wrapfigure}
        {r}{0.47\linewidth}
        \centering
        \resizebox{0.9\linewidth}{!}{\input{AuthorKit25/AnonymousSubmission/LaTeX/plots_lambda.tex}}
        \caption{Analysis of Utility Metric, Gradient Influence Function,
        Hessian weighted Relative Similarity Term, on Different choices of $\lambda
        (t)$ on MNIST Dataset}
    \end{wrapfigure}

    \textbf{Observations} As shown in Figure 5, our batchwise approach significantly
    outperforms all baselines and achieves competitive speed with \cite{killamsetty2023milo}.
    While \cite{killamsetty2023milo} relies on expensive offline preprocessing
    to generate pre-determined subsets for selection during training, our method
    performs online computation, resulting in a slight speed gap. However, as
    demonstrated in the Appendix, this gap is minimal, while our method achieves
    higher accuracy. Please refer to Table \ref{tab:vision_results}. in Appendix
    for detailed evaluations.

    \subsection{Ablation Study results}
    To understand how the choice of submodular function at each step affects the
    model performance under \textbf{Exploration/Exploitation} scheme, it is
    important to understand how the underlying variables affect the overal
    submodular function selection and thereby model performance at each step.

    Here we study the effect of the mixup probability sampling $\lambda(t)$ for
    each step $t$, warm-start, $\pi$ and other hyperparameters. Figure 3a showcases
    the model performance based on the mixup probability. The initial takeaway
    is that as probability of choosing from $\mathcal{B}_{t}$ increases over
    time, the model sees a lot of diverse samples.

    \textbf{Choices for mixup probability $\lambda$ as a constant probability}
    During the case of $\lambda(t) = \epsilon$ (constant probability through out
    the training steps) we take progressively increasing values of the mixup
    probability $\epsilon \in [0.1,0.7]$ as indicated in Figure 3(a) suggest that
    as $\lambda$ value increases, the validation accuracy performances also
    improves.

    \textbf{Decaying Mixup probability}: For emulating a decaying mixup
    probability, we design an exponential decaying function $\lambda(t) = e^{-\mathfrak{j}t}$
    where $j$ is a scalar.

    \textbf{Growing Mixup probability}: Similarly for designing a growing mixup probability
    $\lambda(t) = 1-e^{-\mathfrak{j}t}$

    For both use cases its observed that as the mixup probability samples more
    from the current batch performance improves, but not as linearly as one should
    expect.

    % \subsubsection{Warm-Start}
    % \alertbyPC{Prayas: Check Gchat}
    % For each of the algorithms
    % we consider in this paper (i.e., GRAD-MATCH, GRADMATCHPB, CRAIG, CRAIGPB, and GLISTER), we also
    % consider a warm-start variant, where we run Tf epochs of
    % full training. We set Tf in a way such that the number of
    % epochs Ts with the subset of data is a fraction κ of the total
    % number of epochs, i.e., Ts = κT and Tf =
    % Tsk
    % n
    % , where k
    % is the subset size. We observe that doing full training for
    % the first few epochs helps obtain good warm-start models,
    % resulting in much better convergence.

    % In conjuction with approaches in \cite{killamsetty2021grad} we also conduct experiments using warm-start strategy where we train the model with full batch setting for initial few epochs followed by our strategy. Results for the same are provided in Appendix \ref{Appendix:ExtraDatasets}

    \textbf{Effect of $\pi$} Figure 3(b) showcases that as $\pi$ is progressively
    increased keeping the mixup probability constant, the model performance
    improves which is justified even through our theoretical analysis that as
    $\pi$ is increased, it results in stronger regret bounds.



==> AuthorKit25/AnonymousSubmission/LaTeX/submodularityProof.tex <==
%\subsection{Proof. for submodularity of marginal gain } \textcolor{red}{Remove this proof.}
\iffalse
\begin{theorem}   
The utility function $\boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\mathcal{A}_t;\bullet)$ defined under is \textbf{monotone} and \textbf{submodular} in terms of the set $\mathcal{A}_t$ under certain constraints i.e. $\forall$
$\mathcal{B}_t \subseteq \mathcal{A}_t \subseteq \mathcal{V}$ we have the marginal gain satisfy
    \begin{align*}
    \begin{aligned}
        \boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\boldsymbol{z}_i | \mathcal{B}_t) \geq \boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\boldsymbol{z}_i | \mathcal{A}_t) 
    \end{aligned} 
\end{align*} 
where $\boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\boldsymbol{z}_i | \mathcal{S}) =  \boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\mathcal{S} \cup \{\boldsymbol{z}_i\};\boldsymbol{z}^{\text{val}} ) - \boldsymbol{\boldsymbol{\mathcal{U}}}^{t}(\mathcal{S} ; \boldsymbol{z}^{\text{val}})$ $\forall$ $\mathcal{S} \subseteq \mathcal{V}$
\end{theorem}
\begin{proof}
\textbf{Submodularity}:
\begin{equation}
\begin{split}
\boldsymbol{\boldsymbol{\mathcal{U}}}^t(\boldsymbol{z}_i \mid \mathcal{A}_t) =  \eta_t\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\cdot\boldsymbol{\mathfrak{g}}(\boldsymbol{z}^{\texttt{val}}) - \eta_t^2\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\boldsymbol{\mathfrak{h}}(\boldsymbol{z}^{\texttt{val}})\sum_{\boldsymbol{z} \in \mathcal{A}_t}\boldsymbol{\mathfrak{g}}(\boldsymbol{z})  \\ 
= \eta_t\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\cdot\boldsymbol{\mathfrak{g}}(\boldsymbol{z}^{\texttt{val}}) - \eta_t^2\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\boldsymbol{\mathfrak{h}}(\boldsymbol{z}^{\texttt{val}})\sum_{\boldsymbol{z} \in \mathcal{A}_t \setminus \mathcal{B}_t}\boldsymbol{\mathfrak{g}}(\boldsymbol{z})  
- \eta_t^2\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\boldsymbol{\mathfrak{h}}(\boldsymbol{z}^{\texttt{val}})\sum_{\boldsymbol{z} \in \mathcal{B}_t}\boldsymbol{\mathfrak{g}}(\boldsymbol{z}) \\
=
\boldsymbol{\boldsymbol{\mathcal{U}}}^t(\boldsymbol{z}_i \mid \mathcal{B}_t) - \eta_t^2\boldsymbol{\mathfrak{g}}(\boldsymbol{z}_i)\boldsymbol{\mathfrak{h}}(\boldsymbol{z}^{\texttt{val}})\sum_{\boldsymbol{z} \in \mathcal{A}_t \setminus \mathcal{B}_t}\boldsymbol{\mathfrak{g}}(\boldsymbol{z}) \\
\implies \boldsymbol{\boldsymbol{\mathcal{U}}}^t(\boldsymbol{z}_i \mid \mathcal{B}_t) \geq \boldsymbol{\boldsymbol{\mathcal{U}}}^t(\boldsymbol{z}_i \mid \mathcal{A}_t)\\
\end{split}
\end{equation}
\end{proof}
\fi



==> AuthorKit25/AnonymousSubmission/LaTeX/tables.tex <==
% \definecolor{Silver}{rgb}{0.752,0.752,0.752}
% \begin{table}
% \centering
% \caption{Table of Notations}
% \resizebox{\textwidth}{!}{
% \begin{tblr}{
%   row{odd} = {gray!20},
%   cell{1}{4} = {c=3}{c},
%   cell{1}{7} = {c=3}{c},
%   hlines,
%   vline{1-5,8} = {1}{},
%   vline{-} = {2-16,18-51}{},
%   vline{2-10} = {17}{},
% }
% Dataset  & Model    & Selection Strategy                      & Test accuracy(\%) &        &       & Training time(hrs) &        &        \\
% ~        & ~        & ~                                       & 10\%                                 & 30\%   & 50\%  & 10\%                 & 30\%   & 50\%   \\
% ~        & ~        & ~                                       & ~                                    & ~      &       & ~                    & ~      &        \\
% CIFAR10  & ResNet18 & FULL (skyline for test accuracy)        & 96.12                                & 96.12  &       & 2.37                 & 2.37   &        \\
% ~        & ~        & RANDOM (skyline for training time)      & 80.8                                 & 87.6   &       & 0.46                 & 1.38   &        \\
% ~        & ~        & RANDOM-WARM (skyline for training time) & 87.8                                 & 92.6   &       & 0.42                 & 1.376  &        \\
% ~        & ~        & GLISTER                                 & 91.92                                & 93.63  &       & 0.91                 & 1.46   &        \\
% ~        & ~        & Glister-WArm                            & 91.56                                & 94.09  &       & 0.88                 & 1.40   &        \\
% ~        & ~        & Craig                                   & 87.49                                & 92.53  &       & 1.08                 & 2.399  &        \\
% ~        & ~        & Craig-Warm                              & 89.28                                & 92.82  &       & 0.91                 & 2.20   &        \\
% ~        & ~        & CRAIGb                                 & 88.77                                & 93.58  &       & 0.70                 & 2.07   &        \\
% ~        & ~        & CRAIGb-Warm                            & 90.07                                & 93.8   &       & 0.647                & 2.06   &        \\
% ~        & ~        & GRADMATCH                               & 90.9                                 & 91.89  &       & 0.84                 & 1.52   &        \\
% ~        & ~        & GRADMATCH-Warm                          & 92.15                                & 92.01  &       & 0.73                 & 1.41   &        \\
% ~        & ~        & GRADMATCHPB                             & 90.01                                & 93.75  &       & 0.69                 & 1.38   &        \\
% ~        & ~        & GRADMATCHPb-WARM                        & 92.26                                & 94.17  &       & 0.62                 & 1.36   &        \\
%          &          & RHO-LOSS                                & 87.91                                & 88.49  & 88.49 & 1.14                 & 1.2    & 1.28   \\
%          &          & BOSS                                    & 83.26                                & 91.36  & 91.36 & 0.287                & 0.46   & 0.85   \\
%          &          & $\methodprop$ (ours)                             &                                      &        &       &                      &        &        \\
% CIFAR100 & ResNet18 & FULL (skyline for test accuracy)        & 75.37                                & 75.37  &       & 4.871                & 4.871  &        \\
% ~        & ~        & RANDOM (skyline for training time)      & 31.56                                & 58.56  &       & 0.4699               & 1.453  &        \\
% ~        & ~        & RANDOM-WARM (skyline for training time) & 65.95                                & 72.4   &       & 0.468                & 1.43   &        \\
% ~        & ~        & GLISTER                                 & 44.03                                & 70.49  &       & 0.6456               & 1.5255 &        \\
% ~        & ~        & Glister-WARM                            & 64.95                                & 72.43  &       & 0.6059               & 1.452  &        \\
% ~        & ~        & Craig                                   & 55.19                                & 70.01  &       & 1.785                & 2.654  &        \\
% ~        & ~        & Craig-Warm                              & 67.3                                 & 72.77  &       & 1.48                 & 2.4112 &        \\
% ~        & ~        & CRAIGb                                 & 54.59                                & 70.61  &       & 0.6564               & 1.540  &        \\
% ~        & ~        & CRAIGb-Warm                            & 67.8                                 & 73.79  &       & 0.6030               & 1.5567 &        \\
% ~        & ~        & GRADMATCH                               & 59.88                                & 71.5   &       & 0.8114               & 2.002  &        \\
% ~        & ~        & GRADMATCH-Warm                          & 68.23                                & 74.06  &       & 0.7165               & 1.985  &        \\
% ~        & ~        & GRADMATCHpb                             & 60.39                                & 72.57  &       & 0.6115               & 1.56   &        \\
% ~        & ~        & GRADMATCHPB-WARM                        & 69.58                                & 74.62  &       & 0.5744               & 1.5683 &        \\
%          &          & RHO-LOSS                                & 56                                   & 59.64  & 61    & 1.15                 & 1.15   & 3.18   \\
%          &          & BOSS                                    & 37.68                                & 54.57  & 63.45 & 1.265                & 3.323  & 5.350  \\
%          &          & $\methodprop$ (ours)                             &                                      &        &       &                      &        &        \\
% SVHN     & ResNet18 & FULL (skyline for test accuracy)        & 96.49                                & 96.49  &       & 6.436                & 6.436  &        \\
% ~        & ~        & RANDOM (skyline for training time)      & 93.477                               & 95.31  &       & 0.6383               & 1.90   &        \\
% ~        & ~        & RANDOM-WARM (skyline for training time) & 94.4                                 & 96.01  &       & 0.637                & 1.90   &        \\
% ~        & ~        & GLISTER                                 & 95.37                                & 95.82  &       & 0.9141               & 2.514  &        \\
% ~        & ~        & GLISTER-WARM                            & 95.50                                & 95.69  &       & 0.8522               & 2.34   &        \\
% ~        & ~        & Craig                                   & 94.86                                & 96.223 &       & 1.7566               & 3.177  &        \\
% ~        & ~        & Craig-Warm                              & 95.27                                & 96.15  &       & 1.4599               & 2.6617 &        \\
% ~        & ~        & CRAIGb                                 & 95.367                               & 96.043 &       & 1.069                & 2.413  &        \\
% ~        & ~        & CRAIGb-Warm                            & 95.724                               & 96.385 &       & 0.93406              & 2.332  &        \\
% ~        & ~        & GRADMATCH                               & 94.45                                & 95.73  &       & 1.1541               & 2.981  &        \\
% ~        & ~        & GRADMATCH-Warm                          & 95.13                                & 95.79  &       & 0.9313               & 2.417  &        \\
% ~        & ~        & GRADMATCHipb                            & 95.36                                & 96.24  &       & 0.8438               & 2.52   &        \\
% ~        & ~        & GRADMATCHPB-WARm                        & 95.64                                & 96.425 &       & 0.7889               & 2.398  &        \\
%          &          & RHO-LOSS                                & 94.64                                & 94.27  & 94.85 & 1.08                 & 1.08   & 1.08   \\
%          &          & BOSS                                    & 94.31                                & 95.75  & 96.01 & 0.1774               & 0.7816 & 0.7244 \\
%          &          & $\methodprop$ (ours)                             &                                      &        &       &                      &        &        
% \end{tblr}}
% \end{table}




% \usepackage{color}
% \usepackage{tabularray}
% \usepackage{colortbl}


% % \usepackage{color}
% % \usepackage{tabularray}
% \definecolor{Ebb}{rgb}{0.917,0.901,0.901}
% \begin{table}
% \centering
% \caption{Data selection results}
% \begin{tblr}{
%   row{odd} = {Ebb},
%   row{36} = {Ebb},
%   row{38} = {Ebb},
%   row{40} = {Ebb},
%   row{42} = {Ebb},
%   column{3} = {c},
%   column{4} = {c},
%   column{5} = {c},
%   column{6} = {c},
%   column{7} = {c},
%   column{8} = {c},
%   cell{1}{3} = {c=3}{},
%   cell{1}{6} = {c=3}{},
%   cell{10}{3} = {fg=blue},
%   cell{10}{4} = {fg=red},
%   cell{13}{3} = {fg=red},
%   cell{13}{4} = {fg=blue},
%   cell{20}{3} = {fg=blue},
%   cell{20}{4} = {fg=blue},
%   cell{20}{5} = {fg=blue},
%   cell{23}{3} = {fg=red},
%   cell{23}{4} = {fg=red},
%   cell{23}{5} = {fg=red},
%   hlines,
%   vlines,
% }
% Dataset      & Selection Strategy                      & Test accuracy(\%) &        &       & Training time(hrs) &        &         \\
%              &                                         & 10\%                    & 30\%   & 50\%  & 10\%               & 30\%   & 50\%    \\
%              &                                         &                         &        &       &                    &        &         \\
% CIFAR10      & FULL (skyline for test accuracy)        & 96.12                   & 96.12  & 96.12 & 2.37               & 2.37   & 2.37    \\
%              & RANDOM (skyline for training time)      & 80.8                    & 87.6   & 88.24 & 0.46               & 1.38   & 2.3     \\ 
%              & RANDOM-WARM (skyline for training time) & 87.8                    & 92.6   & 93.1      & 0.42               & 1.376  &    2.24     \\
%              & CRAIGPB                                & 88.77                   & 93.58  &  93.81     & 0.70               & 2.07   &     3.34   \\
%              & CRAIGPB-WARM                           & 90.07                   & 93.8   &  94.32     & 0.647              & 2.06   &   3.26      \\
%              & GRADMATCHPB                             & 90.01                   & 93.75  &   94.12    & 0.69               & 1.38   &     2.06    \\
%              & GRADMATCHPB-WARM                        & 92.26                   & 94.17  &   \textcolor{red}{94.64}    & 0.62               & 1.36   &   1.98      \\
%              & RHO-LOSS                                & 87.91                   & 88.49  & 88.49 & 1.14               & 1.2    & 1.28    \\
%              & BOSS                                    & 83.26                   & 91.36  & \textcolor{blue}{94.53} & 0.287              & 0.46   & 0.85    \\
%              & \textbf{$\methodprop$ (ours)}           & 92.41                   & 93.98  & 94.18 & 0.248              & 0.505  & 0.582   \\
% CIFAR100     & FULL (skyline for test accuracy)        & 75.37                   & 75.37  &   75.37    & 4.871              & 4.871  &  4.871       \\
%              & RANDOM (skyline for training time)      & 31.56                   & 58.56  &  6     & 0.4699             & 1.453  &  2.41       \\
%              & RANDOM-WARM (skyline for training time) & 65.95                   & 72.4   &   73.56    & 0.468              & 1.43   & 2.39        \\
%              & CRAIGPB                                & 54.59                   & 70.61  &  72.24     & 0.6564             & 1.540  &  2.56       \\
%              & CRAIGPB-WARM                           & 67.8                    & 73.79  &   74.46    & 0.6030             & 1.5567 &   2.48      \\
%              & GRADMATCHPB                             & 60.39                   & 72.57  &  73.88     & 0.6115             & 1.56   &    2.53     \\
%              & GRADMATCHPB-WARM                        & 69.58                   & 74.62  & 75.36 & 0.5744             & 1.5683 &       2.51  \\
%              & RHO-LOSS                                & 56                      & 59.64  & 61    & 1.15               & 1.15   & 3.18    \\
%              & BOSS                                    & 37.68                   & 54.57  & 63.45 & 1.265              & 3.323  & 5.350   \\
%              & \textbf{$\methodprop$ (ours)}           & 72.74                   & 74.82  & 75.78 & 0.176              & 0.353  & 0.44055 \\
% % SVHN         & FULL (skyline for test accuracy)        & 96.49                   & 96.49  &    96.49   & 6.436              & 6.436  &  6.436       \\
% %              & RANDOM (skyline for training time)      & 93.477                  & 95.31  &    96.06   & 0.6383             & 1.90   &   3.19      \\
% %              & RANDOM-WARM (skyline for training time) & 94.4                    & 96.01  &   96.24    & 0.637              & 1.90   &   3.18      \\
% %              & CRAIGPB                                & 95.367                  & 96.043 &    96.28   & 1.069              & 2.413  & 4.29        \\
% %              & CRAIGPB-WARM                           & 95.724                  & 96.385 &   96.44    & 0.93406            & 2.332  & 4.17        \\
% %              & GRADMATCHPB                             & 95.36                   & 96.24  &   96.32    & 0.8438             & 2.52   & 4.31        \\
% %              & GRADMATCHPB-WARM                        & 95.64                   & 96.425 &   96.52    & 0.7889             & 2.398  &  4.19       \\
% %              & RHO-LOSS                                & 94.64                   & 94.27  & 94.85 & 1.08               & 1.08   & 1.08    \\
% %              & BOSS                                    & 94.31                   & 95.75  & 96.01 & 0.1774             & 0.7816 & 0.7244  \\
% %              & \textbf{$\methodprop$ (ours)}           &                     95.56    &   96.34     &    96.46   &             0.3123       &   0.6483     &   0.7683      \\
% % TinyImagenet & FULL (skyline for test accuracy)        & 62.14                   & 62.14  & 62.14 & 14.91              & 14.91  & 14.91   \\
% %              & RANDOM (skyline for training time)      & 21.71                   & 36.71  & 41.88 & 1.82               & 4.92   & 10.81   \\
% %              & RANDOM-WARM (skyline for training time) & 26.18                   & 39.44  & 47.61 & 2.07               & 5.11   & 10.93   \\
% %              & CRAIGPB                                & 34.31                   & 41.22  & 49.41 &                    &        &         \\
% %              & CRAIGPB-WARM                           &  35.75                       &  43.63      &  51.38     &                    &        &         \\
% %              & GRADMATCHPB                             &  35.64                       & 50.34       &   54.82    &                    &        &         \\
% %              & GRADMATCHPB-WARM                        &      37.89                   &  53.46      &  56.14     &                    &        &         \\
% %              & RHO-LOSS                                &    41.23                     &  49.61      &   52.89    &                    &        &         \\
% %              & BOSS                                    & 94.31                   & 95.75  & 96.01 & 0.1774             & 0.7816 & 0.7244  \\
% %              & \textbf{$\methodprop$ (ours)}           & 55.96                   & 59.63  & 62.13 & 0.82               & 1.41   & 1.944   
% \end{tblr}
% \end{table}


% \begin{table}
% \centering
% \caption{Table of Notations}
% \begin{tblr}{
%   row{odd} = {Ebb},
%   row{36} = {Ebb},
%   row{38} = {Ebb},
%   row{40} = {Ebb},
%   row{42} = {Ebb},
%   column{3} = {c},
%   column{4} = {c},
%   column{5} = {c},
%   column{6} = {c},
%   column{7} = {c},
%   column{8} = {c},
%   cell{1}{3} = {c=3}{},
%   cell{1}{6} = {c=3}{},
%   % cell{10}{3} = {fg=blue},
%   % cell{10}{4} = {fg=red},
%   % cell{13}{3} = {fg=red},
%   % cell{13}{4} = {fg=blue},
%   % cell{20}{3} = {fg=blue},
%   % cell{20}{4} = {fg=blue},
%   % cell{20}{5} = {fg=blue},
%   % cell{23}{3} = {fg=red},
%   % cell{23}{4} = {fg=red},
%   % cell{23}{5} = {fg=red},
%   hlines,
%   vlines,
% }
% Dataset      & Selection Strategy                      & Test accuracy(\%) &        &       & Training time(hrs) &        &         \\
%              &                                         & 10\%                    & 30\%   & 50\%  & 10\%               & 30\%   & 50\%    \\
%              &                                         &                         &        &       &                    &        &         \\
% % CIFAR10      & FULL (skyline for test accuracy)        & 96.12                   & 96.12  & 96.12 & 2.37               & 2.37   & 2.37    \\
% %              & RANDOM (skyline for training time)      & 80.8                    & 87.6   & 88.24 & 0.46               & 1.38   & 2.3     \\ 
% %              & RANDOM-WARM (skyline for training time) & 87.8                    & 92.6   & 93.1      & 0.42               & 1.376  &    2.24     \\
% %              & CRAIGPB                                & 88.77                   & 93.58  &  93.81     & 0.70               & 2.07   &     3.34   \\
% %              & CRAIGPB-WARM                           & 90.07                   & 93.8   &  94.32     & 0.647              & 2.06   &   3.26      \\
% %              & GRADMATCHPB                             & 90.01                   & 93.75  &   94.12    & 0.69               & 1.38   &     2.06    \\
% %              & GRADMATCHPB-WARM                        & 92.26                   & 94.17  &   94.64    & 0.62               & 1.36   &   1.98      \\
% %              & RHO-LOSS                                & 87.91                   & 88.49  & 88.49 & 1.14               & 1.2    & 1.28    \\
% %              & BOSS                                    & 83.26                   & 91.36  & 94.53 & 0.287              & 0.46   & 0.85    \\
% %              & \textbf{$\methodprop$ (ours)}           & 92.41                   & 93.98  & 94.18 & 0.248              & 0.505  & 0.582   \\
% % CIFAR100     & FULL (skyline for test accuracy)        & 75.37                   & 75.37  &   75.37    & 4.871              & 4.871  &  4.871       \\
% %              & RANDOM (skyline for training time)      & 31.56                   & 58.56  &  6     & 0.4699             & 1.453  &  2.41       \\
% %              & RANDOM-WARM (skyline for training time) & 65.95                   & 72.4   &   73.56    & 0.468              & 1.43   & 2.39        \\
% %              & CRAIGPB                                & 54.59                   & 70.61  &  72.24     & 0.6564             & 1.540  &  2.56       \\
% %              & CRAIGPB-WARM                           & 67.8                    & 73.79  &   74.46    & 0.6030             & 1.5567 &   2.48      \\
% %              & GRADMATCHPB                             & 60.39                   & 72.57  &  73.88     & 0.6115             & 1.56   &    2.53     \\
% %              & GRADMATCHPB-WARM                        & 69.58                   & 74.62  & 75.36 & 0.5744             & 1.5683 &       2.51  \\
% %              & RHO-LOSS                                & 56                      & 59.64  & 61    & 1.15               & 1.15   & 3.18    \\
% %              & BOSS                                    & 37.68                   & 54.57  & 63.45 & 1.265              & 3.323  & 5.350   \\
% %              & \textbf{$\methodprop$ (ours)}           & 72.74                   & 74.82  & 75.78 & 0.176              & 0.353  & 0.44055 \\
% SVHN         & FULL (skyline for test accuracy)        & 96.49                   & 96.49  &    96.49   & 6.436              & 6.436  &  6.436       \\
%              & RANDOM (skyline for training time)      & 93.477                  & 95.31  &    96.06   & 0.6383             & 1.90   &   3.19      \\
%              & RANDOM-WARM (skyline for training time) & 94.4                    & 96.01  &   96.24    & 0.637              & 1.90   &   3.18      \\
%              & CRAIGPB                                & 95.367                  & 96.043 &    96.28   & 1.069              & 2.413  & 4.29        \\
%              & CRAIGPB-WARM                           & \textcolor{red}{95.724}                  & \textcolor{blue}{96.385} &   96.44    & 0.93406            & 2.332  & 4.17        \\
%              & GRADMATCHPB                             & 95.36                   & 96.24  &   96.32    & 0.8438             & 2.52   & 4.31        \\
%              & GRADMATCHPB-WARM                        & \textcolor{blue}{95.64}                   & \textcolor{red}{96.425} &   \textcolor{red}{96.52}    & 0.7889             & 2.398  &  4.19       \\
%              & RHO-LOSS                                & 94.64                   & 94.27  & 94.85 & 1.08               & 1.08   & 1.08    \\
%              & BOSS                                    & 94.31                   & 95.75  & 96.01 & 0.1774             & 0.7816 & 0.7244  \\
%              & \textbf{$\methodprop$ (ours)}           &                     95.56    &   96.34     &    \textcolor{blue}{96.46}   &             0.3123       &   0.6483     &   0.7683      \\
% TinyImagenet & FULL (skyline for test accuracy)        & 62.14                   & 62.14  & 62.14 & 14.91              & 14.91  & 14.91   \\
%              & RANDOM (skyline for training time)      & 21.71                   & 36.71  & 41.88 & 1.82               & 4.92   & 10.81   \\
%              & RANDOM-WARM (skyline for training time) & 26.18                   & 39.44  & 47.61 & 2.07               & 5.11   & 10.93   \\
%              & CRAIGPB                                & 34.31                   & 41.22  & 49.41 &                    &        &         \\
%              & CRAIGPB-WARM                           &  35.75                       &  43.63      &  51.38     &                    &        &         \\
%              & GRADMATCHPB                             &  35.64                       & 50.34       &   54.82    &                    &        &         \\
%              & GRADMATCHPB-WARM                        &      37.89                   &  53.46      &  56.14     &                    &        &         \\
%              & RHO-LOSS                                &    41.23                     &  49.61      &   52.89    &                    &        &         \\
%              & BOSS                                    & 94.31                   & 95.75  & 96.01 & 0.1774             & 0.7816 & 0.7244  \\
%              & \textbf{$\methodprop$ (ours)}           & \textcolor{red}{55.96}                   & \textcolor{red}{59.63}  & \textcolor{red}{62.13} & 0.82               & 1.41   & 1.944   
% \end{tblr}
% \end{table}




% \usepackage{color}
% \usepackage{tabularray}
% \documentclass{article}
% \usepackage{amsmath}
% \usepackage{xcolor}
% \usepackage{tabularray}
% \usepackage{threeparttable}
% \begin{document}

% \begin{table}
% \centering
% \caption{Data Selection Results on Vision Datasets}
% \label{tab:vision_results}
% \begin{tblr}{
%   colspec = {Q[c]Q[c]Q[c]Q[c]Q[c]Q[c]Q[c]Q[c]}, % Explicit column spec
%   hline{1,21} = {-}{0.08em},
%   hline{2} = {2-8}{},
% hline{2, 30} = {-}{},
% hline{3,12} = {-}{0.05em},
% }
% \textbf{Dataset}      & \textbf{Selection Strategy}             & \SetCell[c=3]{c}\textbf{Test accuracy (\%)} &                &                & \SetCell[c=3]{c}\textbf{Training time (hrs)}&       &       \\
%                       &                  Budget(\%)                      & 10\%                        & 30\%           & 50\%           & 10\%                         & 30\%  & 50\%  \\
% \textbf{CIFAR10}      & FULL (skyline for test accuracy)        & 96.12                   & 96.12  & 96.12 & 2.37               & 2.37   & 2.37    \\
%              & RANDOM (skyline for training time)      & 80.8                    & 87.6   & 88.24 & 0.46               & 1.38   & 2.3     \\ 
%              & CRAIGPB                                & 88.77                   & 93.58  &  93.81     & 0.70               & 2.07   &     3.34   \\
%              & CRAIGPB-WARM                           & 90.07                   & 93.8   &  94.32     & 0.647              & 2.06   &   3.26      \\
%              & GRADMATCHPB                             & 90.01                   & 93.75  &   94.12    & 0.69               & 1.38   &     2.06    \\
%              & GRADMATCHPB-WARM                        & \textcolor{blue}{92.26}                   & \textcolor{red}{94.17}  &   \textcolor{red}{94.64}    & 0.62               & 1.36   &   1.98      \\
%              & RHO-LOSS                                & 87.91                   & 88.49  & 88.49 & 1.14               & 1.2    & 1.28    \\
%              & BOSS                                    & 83.26                   & 91.36  & \textcolor{blue}{94.53} & 0.287              & 0.46   & 0.85    \\
%              & \textbf{$\methodprop$ (ours)}           & \textcolor{red}{92.41}                   & \textcolor{blue}{93.98}  & 94.18 & 0.248              & 0.505  & 0.582   \\
% \textbf{CIFAR100}     & FULL (skyline for test accuracy)        & 75.37                   & 75.37  &   75.37    & 4.871              & 4.871  &  4.871       \\
%              & RANDOM (skyline for training time)      & 31.56                   & 58.56  &  60.67     & 0.4699             & 1.453  &  2.41       \\
%              & CRAIGPB                                & 54.59                   & 70.61  &  72.24     & 0.6564             & 1.540  &  2.56       \\
%              & CRAIGPB-WARM                           & 67.8                    & 73.79  &   74.46    & 0.6030             & 1.5567 &   2.48      \\
%              & GRADMATCHPB                             & 60.39                   & 72.57  &  73.88     & 0.6115             & 1.56   &    2.53     \\
%              & GRADMATCHPB-WARM                        & \textcolor{blue}{69.58}                   & \textcolor{blue}{74.62}  & \textcolor{blue}{75.36} & 0.5744             & 1.5683 &       2.51  \\
%              & RHO-LOSS                                & 56                      & 59.64  & 61    & 1.15               & 1.15   & 3.18    \\
%              & BOSS                                    & 37.68                   & 54.57  & 63.45 & 1.265              & 3.323  & 5.350   \\
%              & \textbf{$\methodprop$ (ours)}           & \textcolor{red}{72.74}                   & \textcolor{red}{74.82}  & \textcolor{red}{75.78} & 0.176              & 0.353  & 0.4405 \\
% \textbf{SVHN}         & FULL (skyline for test accuracy)        & 96.49                   & 96.49  &    96.49   & 6.436              & 6.436  &  6.436       \\
%              & RANDOM (skyline for training time)      & 93.477                  & 95.31  &    96.06   & 0.6383             & 1.90   &   3.19      \\
             
%              & CRAIGPB                                & 95.367                  & 96.043 &    96.28   & 1.069              & 2.413  & 4.29        \\
%              & CRAIGPB-WARM                           & \textcolor{red}{95.724}                  & \textcolor{blue}{96.385} &   96.44    & 0.93406            & 2.332  & 4.17        \\
%              & GRADMATCHPB                             & 95.36                   & 96.24  &   96.32    & 0.8438             & 2.52   & 4.31        \\
%              & GRADMATCHPB-WARM                        & \textcolor{blue}{95.64}                   & \textcolor{red}{96.425} &   \textcolor{red}{96.52}    & 0.7889             & 2.398  &  4.19       \\
%              & RHO-LOSS                                & 94.64                   & 94.27  & 94.85 & 1.08               & 1.08   & 1.08    \\
%              & BOSS                                    & 94.31                   & 95.75  & 96.01 & 0.1774             & 0.7816 & 0.7244  \\
%              & \textbf{$\methodprop$ (ours)}           &                     95.56    &   96.34     &    \textcolor{blue}{96.46}   &             0.3123       &   0.6483     &   0.7683      \\
% \textbf{TinyImagenet} & FULL (skyline for test accuracy)        & 62.14                   & 62.14  & 62.14 & 14.91              & 14.91  & 14.91   \\
%              & RANDOM (skyline for training time)      & 21.71                   & 36.71  & 41.88 & 1.82               & 4.92   & 10.81   \\
             
%              & CRAIGPB                                & 34.31                   & 41.22  & 49.41 &         &   &         \\
%              & CRAIGPB-WARM                           &  35.75                       &  43.63      &  51.38     &         &   &         \\
%              & GRADMATCHPB                             &  35.64                       & 50.34       &   54.82    &         &   &         \\
%              & GRADMATCHPB-WARM                        &      37.89                   &  53.46      &  56.14     &         &   &         \\
%              & RHO-LOSS                                &    41.23                     &  49.61      &   52.89    &         &   &         \\
%              & BOSS                                    & 32.54                   & 51.21  & 57.77 & 1.2             & 2.11 & 3.16  \\
%              & \textbf{$\methodprop$ (ours)}           & \textcolor{red}{55.96}                   & \textcolor{red}{59.63}  & \textcolor{red}{62.13} & 0.82               & 1.41   & 1.944   


% \end{tblr}


% \end{table}

% \end{document}


% #################### PERBATCH TABLE ####################



